An Introduction to Double/Debiased Machine Learning

This paper provides an introduction to Double/Debiased Machine Learning (DML). DML is a general approach to performing inference about a target parameter in the presence of nuisance functions: objects that are needed to identify the target parameter but are not of primary interest. Nuisance functions arise naturally in many settings, such as when controlling for confounding variables or leveraging instruments. The paper describes two biases that arise from nuisance function estimation and explains how DML alleviates these biases. Consequently, DML allows the use of flexible methods, including machine learning tools, for estimating nuisance functions, reducing the dependence on auxiliary functional form assumptions and enabling the use of complex non-tabular data, such as text or images. We illustrate the application of DML through simulations and empirical examples. We conclude with a discussion of recommended practices. A companion website includes additional examples with code and references to other resources.

==> application_AE/artificialIV_dgp1.tex <==
&First stage&.0004&.0004&.0005&.0035&-.0014&.0004&-.0014 \tabularnewline
&&(.011)&(.011)&(.0109)&(.0127)&(.0055)&(.011)&(.0055) \tabularnewline
&Index&-&0&.0012&.0127&.0092&.0002&.0092 \tabularnewline
&&(-)&(0)&(0)&(.0246)&(.0003)&(.0005)&(.0003) \tabularnewline
&Employment&--2.6761&1.1148&2.481&1.1053&-.8519&6.8049&-.655 \tabularnewline
&&(68.4474)&(35.1599)&(30.8941)&(19.6774)&(21.7516)&(140.802)&(19.196) \tabularnewline
&Weeks worked&--119.6848&33.8069&80.3055&36.4932&--83.1191&292.5573&--61.3623 \tabularnewline
&&(2864.082)&(3084.742)&(1277.043)&(514.9237)&(754.2967)&(6046.517)&(1154.677) \tabularnewline


==> application_AE/artificialIV_dgp1_all.tex <==
&First stage&.0004&.0004&.0005&.0035&-.0014&.0004&-.0014 \tabularnewline
&&(.011)&(.011)&(.0109)&(.0127)&(.0055)&(.011)&(.0055) \tabularnewline
&Index&-&0&.0012&.0127&.0092&.0002&.0092 \tabularnewline
&&(-)&(0)&(0)&(.0246)&(.0003)&(.0005)&(.0003) \tabularnewline
&Employment&--2.6761&1.1148&2.481&1.1053&-.8519&6.8049&-.655 \tabularnewline
&&(68.4474)&(35.1599)&(30.8941)&(19.6774)&(21.7516)&(140.802)&(19.196) \tabularnewline
&Weeks worked&--119.6848&33.8069&80.3055&36.4932&--83.1191&292.5573&--61.3623 \tabularnewline
&&(2864.082)&(3084.742)&(1277.043)&(514.9237)&(754.2967)&(6046.517)&(1154.677) \tabularnewline


==> application_AE/artificialIV_dgp1_all_pres.tex <==
First stage&.0004&.0004&.0005&.0035&-.0014&.0004&-.0014 \tabularnewline
&(.011)&(.011)&(.0109)&(.0127)&(.0055)&(.011)&(.0055) \tabularnewline
Employment&--2.6761&1.1148&2.481&1.1053&-.8519&6.8049&-.655 \tabularnewline
&(68.4474)&(35.1599)&(30.8941)&(19.6774)&(21.7516)&(140.802)&(19.196) \tabularnewline


==> application_AE/artificialIV_dgp1_pres.tex <==
First stage&.0004&.0004&.0005&.0035&-.0014&.0004&-.0014 \tabularnewline
&(.011)&(.011)&(.0109)&(.0127)&(.0055)&(.011)&(.0055) \tabularnewline
Employment&--2.6761&1.1148&2.481&1.1053&-.8519&6.8049&-.655 \tabularnewline
&(68.4474)&(35.1599)&(30.8941)&(19.6774)&(21.7516)&(140.802)&(19.196) \tabularnewline


==> application_AE/artificialIV_dgp2.tex <==
&First stage&.0828&.0828&.0828&.0723&.0435&.0827&.0235 \tabularnewline
&&(.0104)&(.0104)&(.0104)&(.0208)&(.0059)&(.0105)&(.0057) \tabularnewline
&Index&-&0&.0012&.0134&.0093&.0003&.0093 \tabularnewline
&&(-)&(0)&(0)&(.0248)&(.0003)&(.0009)&(.0003) \tabularnewline
&Employment&-.1119&-.1116&-.1039&.0235&-.1036&-.1119&-.1338 \tabularnewline
&&(.1277)&(.1285)&(.1284)&(.3045)&(.1368)&(.1272)&(.2435) \tabularnewline
&Weeks worked&--5.2283&--5.2204&--4.7685&2.3651&-.7736&--5.1799&1.7544 \tabularnewline
&&(5.6945)&(5.7035)&(5.711)&(16.5527)&(6.3336)&(5.691)&(11.6248) \tabularnewline


==> application_AE/artificialIV_dgp2_all.tex <==
&First stage&.0828&.0828&.0828&.0723&.0435&.0827&.0235 \tabularnewline
&&(.0104)&(.0104)&(.0104)&(.0208)&(.0059)&(.0105)&(.0057) \tabularnewline
&Index&-&0&.0012&.0134&.0093&.0003&.0093 \tabularnewline
&&(-)&(0)&(0)&(.0248)&(.0003)&(.0009)&(.0003) \tabularnewline
&Employment&-.1119&-.1116&-.1039&.0235&-.1036&-.1119&-.1338 \tabularnewline
&&(.1277)&(.1285)&(.1284)&(.3045)&(.1368)&(.1272)&(.2435) \tabularnewline
&Weeks worked&--5.2283&--5.2204&--4.7685&2.3651&-.7736&--5.1799&1.7544 \tabularnewline
&&(5.6945)&(5.7035)&(5.711)&(16.5527)&(6.3336)&(5.691)&(11.6248) \tabularnewline


==> application_AE/artificialIV_dgp2_all_pres.tex <==
First stage&.0828&.0828&.0828&.0723&.0435&.0827&.0235 \tabularnewline
&(.0104)&(.0104)&(.0104)&(.0208)&(.0059)&(.0105)&(.0057) \tabularnewline
Employment&-.1119&-.1116&-.1039&.0235&-.1036&-.1119&-.1338 \tabularnewline
&(.1277)&(.1285)&(.1284)&(.3045)&(.1368)&(.1272)&(.2435) \tabularnewline


==> application_AE/artificialIV_dgp2_pres.tex <==
First stage&.0828&.0828&.0828&.0723&.0435&.0827&.0235 \tabularnewline
&(.0104)&(.0104)&(.0104)&(.0208)&(.0059)&(.0105)&(.0057) \tabularnewline
Employment&-.1119&-.1116&-.1039&.0235&-.1036&-.1119&-.1338 \tabularnewline
&(.1277)&(.1285)&(.1284)&(.3045)&(.1368)&(.1272)&(.2435) \tabularnewline


==> application_AE/artificialIV_dgp3.tex <==
&First stage&.0693&.0693&.0693&.0693&.0692&.0693&4.122 \tabularnewline
&&(.0066)&(.0066)&(.0066)&(.0066)&(.0068)&(.0066)&(2.6612) \tabularnewline
&Index&-&0&-.0004&-.0003&0&-.0002&0 \tabularnewline
&&(-)&(0)&(.0005)&(.0004)&(.0003)&(.0003)&(.0001) \tabularnewline
&Employment&-.1286&-.1284&-.1302&-.1311&-.1294&-.1297&-.1849 \tabularnewline
&&(.0987)&(.0989)&(.0988)&(.099)&(.102)&(.0982)&(.7653) \tabularnewline
&Weeks worked&--5.6163&--5.6012&--5.6427&--5.7021&--5.6943&--5.6571&--7.9362 \tabularnewline
&&(4.2916)&(4.3211)&(4.3184)&(4.3223)&(4.3898)&(4.279)&(30.4164) \tabularnewline


==> application_AE/artificialIV_dgp3_all.tex <==
&First stage&.0693&.0693&.0693&.0693&.0692&.0693&4.122 \tabularnewline
&&(.0066)&(.0066)&(.0066)&(.0066)&(.0068)&(.0066)&(2.6612) \tabularnewline
&Index&-&0&-.0004&-.0003&0&-.0002&0 \tabularnewline
&&(-)&(0)&(.0005)&(.0004)&(.0003)&(.0003)&(.0001) \tabularnewline
&Employment&-.1286&-.1284&-.1302&-.1311&-.1294&-.1297&-.1849 \tabularnewline
&&(.0987)&(.0989)&(.0988)&(.099)&(.102)&(.0982)&(.7653) \tabularnewline
&Weeks worked&--5.6163&--5.6012&--5.6427&--5.7021&--5.6943&--5.6571&--7.9362 \tabularnewline
&&(4.2916)&(4.3211)&(4.3184)&(4.3223)&(4.3898)&(4.279)&(30.4164) \tabularnewline


==> application_AE/artificialIV_dgp3_all_pres.tex <==
First stage&.0693&.0693&.0693&.0693&.0692&.0693&4.122 \tabularnewline
&(.0066)&(.0066)&(.0066)&(.0066)&(.0068)&(.0066)&(2.6612) \tabularnewline
Employment&-.1286&-.1284&-.1302&-.1311&-.1294&-.1297&-.1849 \tabularnewline
&(.0987)&(.0989)&(.0988)&(.099)&(.102)&(.0982)&(.7653) \tabularnewline


==> application_AE/artificialIV_dgp3_pres.tex <==
First stage&.0693&.0693&.0693&.0693&.0692&.0693&4.122 \tabularnewline
&(.0066)&(.0066)&(.0066)&(.0066)&(.0068)&(.0066)&(2.6612) \tabularnewline
Employment&-.1286&-.1284&-.1302&-.1311&-.1294&-.1297&-.1849 \tabularnewline
&(.0987)&(.0989)&(.0988)&(.099)&(.102)&(.0982)&(.7653) \tabularnewline


==> application_AE/dgp_linear.tex <==
0&&0.048&0.048&0.065&0.048&0.009&&1.159&1.154&1.180&&0.993&0.993&0.980 \tabularnewline
.01&&0.174&0.166&0.102&0.166&0.028&&0.685&0.693&0.966&&0.990&0.988&0.980 \tabularnewline
.025&&0.776&0.768&0.422&0.768&0.192&&0.281&0.287&0.447&&0.966&0.964&0.976 \tabularnewline
.05&&1.\phantom{000}&1.\phantom{000}&0.984&1.\phantom{000}&0.836&&0.135&0.135&0.152&&0.962&0.960&0.960 \tabularnewline
.075&&1.\phantom{000}&1.\phantom{000}&1.\phantom{000}&1.\phantom{000}&0.992&&0.088&0.088&0.094&&0.956&0.954&0.948 \tabularnewline
.1&&1.\phantom{000}&1.\phantom{000}&1.\phantom{000}&1.\phantom{000}&0.998&&0.067&0.065&0.066&&0.956&0.952&0.950 \tabularnewline


==> application_AE/dgp_linear_pres.tex <==
0&&0.048&0.048&0.009&&1.159&1.154&&0.993&0.993 \tabularnewline
.01&&0.174&0.166&0.028&&0.685&0.693&&0.990&0.988 \tabularnewline
.025&&0.776&0.768&0.192&&0.281&0.287&&0.966&0.964 \tabularnewline
.05&&1.\phantom{000}&1.\phantom{000}&0.836&&0.135&0.135&&0.962&0.960 \tabularnewline
.075&&1.\phantom{000}&1.\phantom{000}&0.992&&0.088&0.088&&0.956&0.954 \tabularnewline
.1&&1.\phantom{000}&1.\phantom{000}&0.998&&0.067&0.065&&0.956&0.952 \tabularnewline


==> application_AE/dgp_linear_vsmall.tex <==
0&&0.048&0.048&&1.159&1.154&&0.993&0.993 \tabularnewline
.01&&0.174&0.166&&0.685&0.693&&0.990&0.988 \tabularnewline
.025&&0.776&0.768&&0.281&0.287&&0.966&0.964 \tabularnewline
.05&&1.\phantom{000}&1.\phantom{000}&&0.135&0.135&&0.962&0.960 \tabularnewline
.075&&1.\phantom{000}&1.\phantom{000}&&0.088&0.088&&0.956&0.954 \tabularnewline
.1&&1.\phantom{000}&1.\phantom{000}&&0.067&0.065&&0.956&0.952 \tabularnewline


==> application_AE/dgp_xgb.tex <==
0&&0.038&0.038&0.097&0.038&0.013&&1.076&1.089&0.945&&0.990&0.993&0.980 \tabularnewline
.01&&0.213&0.215&0.086&0.215&0.042&&0.692&0.667&1.023&&0.980&0.983&0.995 \tabularnewline
.025&&0.805&0.795&0.449&0.795&0.263&&0.282&0.279&0.462&&0.961&0.963&0.971 \tabularnewline
.05&&1.\phantom{000}&1.\phantom{000}&0.980&1.\phantom{000}&0.890&&0.130&0.136&0.155&&0.958&0.961&0.963 \tabularnewline
.075&&1.\phantom{000}&1.\phantom{000}&1.\phantom{000}&1.\phantom{000}&0.995&&0.083&0.085&0.098&&0.946&0.946&0.956 \tabularnewline
.1&&1.\phantom{000}&1.\phantom{000}&1.\phantom{000}&1.\phantom{000}&1.\phantom{000}&&0.065&0.066&0.074&&0.956&0.951&0.949 \tabularnewline


==> application_AE/dgp_xgb_pres.tex <==
0&&0.038&0.038&0.013&&1.076&1.089&&0.990&0.993 \tabularnewline
.01&&0.213&0.215&0.042&&0.692&0.667&&0.980&0.983 \tabularnewline
.025&&0.805&0.795&0.263&&0.282&0.279&&0.961&0.963 \tabularnewline
.05&&1.\phantom{000}&1.\phantom{000}&0.890&&0.130&0.136&&0.958&0.961 \tabularnewline
.075&&1.\phantom{000}&1.\phantom{000}&0.995&&0.083&0.085&&0.946&0.946 \tabularnewline
.1&&1.\phantom{000}&1.\phantom{000}&1.\phantom{000}&&0.065&0.066&&0.956&0.951 \tabularnewline


==> application_AE/dgp_xgb_vsmall.tex <==
0&&0.038&0.038&&1.076&1.089&&0.990&0.993 \tabularnewline
.01&&0.213&0.215&&0.692&0.667&&0.980&0.983 \tabularnewline
.025&&0.805&0.795&&0.282&0.279&&0.961&0.963 \tabularnewline
.05&&1.\phantom{000}&1.\phantom{000}&&0.130&0.136&&0.958&0.961 \tabularnewline
.075&&1.\phantom{000}&1.\phantom{000}&&0.083&0.085&&0.946&0.946 \tabularnewline
.1&&1.\phantom{000}&1.\phantom{000}&&0.065&0.066&&0.956&0.951 \tabularnewline


==> application_AE/pysw.tex <==
OLS&.401&.321&.449&.223&.832&.842 \tabularnewline
CV-Lasso&.365&.374&.26&.281&.144&.128 \tabularnewline
CV-Ridge&.014&.027&.018&.415&.022&.029 \tabularnewline
XGBoost-c&.22&.278&.273&.082&.001&.002 \tabularnewline


==> iv_simulation/jel_linear_results.tex <==
& Mean & Median & SD & Coverage \\
1. 2SLS w/all IVs & 0.3228 & 0.3199 & 0.0447 & 0.0000 \\
2. Stacking, no crossfit & 0.0954 & 0.0978 & 0.0831 & 0.6090 \\
3. DML-FIV, OLS as single learner & -0.0325 & -0.0172 & 0.1725 & 0.9380 \\
4. DML-FIV, Short-stacking & -0.0009 & 0.0059 & 0.0811 & 0.9560 \\ \hline
5. Infeasible IV & -0.0076 & -0.0036 & 0.0773 & 0.9570 \\


==> iv_simulation/jel_stacking_weights.tex <==
& ML (stacking) w/o crossfiting & DML with stacking \\
OLS & 0.0243 & 0.0247 \\
Lasso-CV & 0.4577 & 0.4525 \\
Ridge-CV & 0.4179 & 0.4108 \\
Gradboost, low reg & 0.0401 & 0.0474 \\
Gradboost, high reg & 0.0600 & 0.0646 \\


==> iv_simulation/linear_results.tex <==
& Mean & Median & SD & Coverage \\
1.  Infeasible IV & -0.0076 & -0.0036 & 0.0773 & 0.9570 \\
2.  2SLS w/all IVs & 0.3228 & 0.3199 & 0.0447 & 0.0000 \\
3.  Ridge, no crossfit & 0.0456 & 0.0428 & 0.0904 & 0.8170 \\
4.  Gradboost w/low-reg, no crossfit & 0.3738 & 0.3751 & 0.0370 & 0.0000 \\
5.  Gradboost w/high-reg, no crossfit & 0.1502 & 0.1520 & 0.0580 & 0.2790 \\
6.  Stacking, no crossfit & 0.0954 & 0.0978 & 0.0831 & 0.6090 \\
7.  DML-FIV, OLS as single learner & -0.0325 & -0.0172 & 0.1725 & 0.9380 \\
8.  DML-FIV, ridge as single learner & -0.0131 & -0.0058 & 0.0856 & 0.9550 \\
9.  DML-FIV, Gradboost w/low-reg as single learner & -0.0201 & -0.0051 & 0.1075 & 0.9590 \\
10. DML-FIV, Gradboost w/high-reg as single learner & -0.0159 & -0.0076 & 0.0924 & 0.9590 \\
10. DML-FIV, Short-stacking & -0.0009 & 0.0059 & 0.0811 & 0.9560 \\


==> iv_simulation/nonlinear_results.tex <==
& Mean & Median & SD & Coverage \\
1.  Infeasible IV & -0.0031 & 0.0023 & 0.0819 & 0.9440 \\
2.  2SLS w/all IVs & 0.5162 & 0.5159 & 0.0564 & 0.0000 \\
3.  Ridge, no crossfit & 0.5155 & 0.5129 & 0.0947 & 0.0050 \\
4.  Gradboost w/low-reg, no crossfit & 0.4236 & 0.4227 & 0.0387 & 0.0000 \\
5.  Gradboost w/high-reg, no crossfit & 0.2745 & 0.2739 & 0.0684 & 0.0450 \\
6.  Stacking, no crossfit & 0.4020 & 0.4033 & 0.0451 & 0.0000 \\
7.  DML-FIV, OLS as single learner & -0.6583 & 0.5125 & 29.8626 & 0.9250 \\
8.  DML-FIV, ridge as single learner & 0.7406 & 0.5890 & 13.2413 & 0.9150 \\
9.  DML-FIV, Gradboost w/low-reg as single learner & -0.0268 & 0.0004 & 0.1794 & 0.9540 \\
10. DML-FIV, Gradboost w/high-reg as single learner & -0.0450 & -0.0128 & 0.1983 & 0.9600 \\
10. DML-FIV, Short-stacking & -0.0057 & 0.0102 & 0.1517 & 0.9410 \\


==> iv_simulation/stacking_weights.tex <==
& Linear DGP w/o crossfit & Linear DGP, DML & Nonlinear DGP w/o crosffit & Nonlinear DGP, DML \\
OLS & 0.0243 & 0.0247 & 0.0114 & 0.0103 \\
Lasso-CV & 0.4577 & 0.4525 & 0.0375 & 0.0154 \\
Ridge-CV & 0.4179 & 0.4108 & 0.0116 & 0.0025 \\
Gradboost, low reg & 0.0401 & 0.0474 & 0.5372 & 0.5231 \\
Gradboost, high reg & 0.0600 & 0.0646 & 0.4023 & 0.4487 \\


==> partialinput.tex <==
\makeatletter
\newread\pin@file
\newcounter{pinlineno}
\newcommand\pin@accu{}
\newcommand\pin@ext{pintmp}
% inputs #3, selecting only lines #1 to #2 (inclusive)
\newcommand*\partialinput [3] {%
\IfFileExists{#3}{%
\openin\pin@file #3%
% skip lines 1 to #1 (exclusive)
\setcounter{pinlineno}{1}%
\@whilenum\value{pinlineno}<#1 \do{%
\read\pin@file to\pin@line%
\stepcounter{pinlineno}%
}%
% prepare reading lines #1 to #2 inclusive
\addtocounter{pinlineno}{-1}%
\let\pin@accu\empty%
\begingroup%
\endlinechar\newlinechar
\@whilenum\value{pinlineno}<#2 \do{%
% use safe catcodes provided by e-TeX's \readline
\readline\pin@file to\pin@line%
\edef\pin@accu{\pin@accu\pin@line}%
\stepcounter{pinlineno}%
}%
\closein\pin@file%
\expandafter\endgroup%
\scantokens\expandafter{\pin@accu}%
}{%
\errmessage{File `#3' doesn't exist!}%
}%
}
\makeatother


==> tables/401k/ate_estimates.tex <==
\begin{tabular}{lcccccc}
\toprule
\midrule
& $\check{\theta}_{IPW}^{\dagger,ate}$ & $\check{\theta}_{REG}^{\dagger,ate}$ & $\check{\theta}^{*,ate}$ & $\hat{\theta}_{IPW}^{\dagger,ate}$ & $\hat{\theta}_{REG}^{\dagger,ate}$ & $\hat{\theta}^{*,ate}$ \\ \midrule
& 6289.0 & 7877.8 & 7052.4 & 7456.7 & 7741.3 & 6790.8 \\
& (1222.9) & (183.8) & (587.8) & (1315.5) & (143.3) & (760.2) \\
& & & & & & \\
Neyman orthogonal & No & No & Yes & No & No & Yes \\
Cross-fitting & No & No & No & Yes & Yes & Yes \\
\midrule
\bottomrule
\end{tabular}


==> tables/401k/combined.tex <==
\begin{tabular}{lcccccc}
\toprule
\midrule
& \multicolumn{5}{c}{\it Invalid Estimators}  &{\it DML}\\
\cmidrule(lr){2-6} \cmidrule(lr){7-7}
& $\check{\theta}_{IPW}$ & $\check{\theta}_{RA}$ & $\check{\theta}_{DR}$ & $\hat{\theta}_{IPW}$ & $\hat{\theta}_{RA}$ & $\hat{\theta}_{DR}$ \\ \midrule

\textit{Panel A: SIPP Estimates}& & & & & &\\
& 6289.0 & 7877.8 & 7052.4 & 7456.7 & 7741.3 & 6790.8 \\
& (1222.9) & (183.8) & (587.8) & (1315.5) & (143.3) & (760.2) \\
& & & & \\
\textit{Panel B: Simulation Results}& & & & & &\\
Mean Bias & 747.3 & 644.0 & 142.0 & 756.4 & 594.9 & 47.3 \\
Median Bias & 745.6 & 647.1 & 154.7 & 755.1 & 597.8 & 60.8 \\
Median Abs.\ Deviation & 804.6 & 669.7 & 433.3 & 809.2 & 628.6 & 424.3 \\
Std.\ Deviation & 837.3 & 604.7 & 619.2 & 841.7 & 606.2 & 627.4 \\
Mean Standard Error & 1159.2 & 136.5 & 555.2 & 1171.4 & 125.3 & 617.9 \\
Coverage Rate (0.95) & 0.965 & 0.203 & 0.911 & 0.966 & 0.200 & 0.945 \\
& & & & & & \\
\textit{Panel C: Essential Components}& & & & & &\\
Neyman orthogonal & No & No & Yes & No & No & Yes \\
Cross-fitting & No & No & No & Yes & Yes & Yes \\
\midrule
\bottomrule
\end{tabular}

==> tables/401k/results.tex <==
\begin{tabular}{lcccccc}
\toprule
\midrule
& $\check{\theta}_{IPW}^{\dagger,ATE}$ & $\check{\theta}_{REG}^{\dagger,ATE}$ & $\check{\theta}^{*,ATE}$ & $\hat{\theta}_{IPW}^{\dagger,ATE}$ & $\hat{\theta}_{REG}^{\dagger,ATE}$ & $\hat{\theta}^{*,ATE}$ \\ \midrule
Mean Bias & 747.3 & 644.0 & 142.0 & 756.4 & 594.9 & 47.3 \\
Median Bias & 745.6 & 647.1 & 154.7 & 755.1 & 597.8 & 60.8 \\
Median Abs.\ Deviation & 804.6 & 669.7 & 433.3 & 809.2 & 628.6 & 424.3 \\
Std.\ Deviation & 837.3 & 604.7 & 619.2 & 841.7 & 606.2 & 627.4 \\
Mean Std.\ Error & 1159.2 & 136.5 & 555.2 & 1171.4 & 125.3 & 617.9 \\
Coverage Rate (0.95) & 0.965 & 0.203 & 0.911 & 0.966 & 0.200 & 0.945 \\
& & & & & & \\
Neyman orthogonal & No & No & Yes & No & No & Yes \\
Cross-fitting & No & No & No & Yes & Yes & Yes \\
\midrule
\bottomrule
\end{tabular}


==> tables/GN_2021_dml.tex <==
\resizebox{\linewidth}{!}{\begin{tabular}{l c c c c c c}
\toprule\toprule
 & \multicolumn{6}{c}{\it DML}\\
 \cmidrule{3-7}
 & \multicolumn{6}{c}{\it Candidate learners}\\
 \cmidrule{4-7}
 & (1) & (2) & (3) & (4) & (5) & (6) \\
     & G-N (2021) & Short- & \multirow{2}{*}{Cross-fit OLS} & \multirow{2}{*}{CV-lasso} &  \multirow{2}{*}{Bagging} & Kernel \\
 & OLS & stacking &  &  & & regression \\
\midrule
\multicolumn{8}{l}{\it Panel A. Median coefficient estimates} \\
~~Climatic instability      & $-1.824$ & $-1.671$ & $-1.822$ & $-1.787$ & $-2.020$ & $-1.614$ \\
                  & $(0.696)$      & $(0.701)$      & $(0.683)$      & $(0.804)$      & $(0.787)$      & $(0.708)$      \\
\midrule
\midrule
\multicolumn{8}{l}{\it Panel B. Short-stacking weights for each candidate learner} \\
~~Outcome (importance of tradition)   &             & n/a       & $0.000$       & $0.000$        & $0.000$       & $1.000$        \\
~~Treatment (climatic instability) &             & n/a        & $0.000$        & $0.000$       & $0.151$        & $0.849$        \\
\bottomrule\bottomrule 
\end{tabular}}





==> tables/hrs/attgt_bylearner.tex <==
\begin{tabular}{ccccccccc}
\toprule
\midrule
\makecell{Wave first \\ hospitalized} & Wave & \makecell{Short- \\ stacking} & \makecell{Linear \\ index} & Lasso & Ridge & \makecell{Random \\ Forest (hr)} & \makecell{Random \\ Forest (mr)} & \makecell{Random \\ Forest (lr)}
 \\
      &       & (1)   & (2)   & (3)   & (4)   & (5)   & (6) & (7) \\ \midrule
\multirow{8}[0]{*}{8} & \multirow{2}[0]{*}{7} & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
      &       & - & - & - & - & - & - & - \\
      & \multirow{2}[0]{*}{8} & 2521 & 2272.3 & 2278.3 & 2353.9 & 2470.8 & 2478 & 2480 \\
      &       & (799.6) & (848.6) & (852) & (834) & (805.9) & (798.8) & (800) \\
      & \multirow{2}[0]{*}{9} & 534.3 & 43.3 & 772.7 & 721.5 & 744.9 & 519.9 & 404.4 \\
      &       & (592.6) & (737.2) & (622.6) & (635.5) & (560.2) & (602.8) & (649.1) \\
      & \multirow{2}[0]{*}{10} & 685 & 898.8 & 872.6 & 856.8 & 769.6 & 723.7 & 623.6 \\
      &       & (603) & (638.1) & (518) & (519.2) & (588.5) & (599.9) & (626.8) \\
& & & & & & & & \\
\multirow{8}[0]{*}{9} & \multirow{2}[0]{*}{7} & 930.9 & 1598.6 & 966.1 & 1082.2 & 908.6 & 1358.5 & 1435.1 \\
      &       & (1149) & (1436.2) & (1157.5) & (1299.6) & (986.2) & (994.1) & (978.8) \\
      & \multirow{2}[0]{*}{8} & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
      &       & - & - & - & - & - & - & - \\
      & \multirow{2}[0]{*}{9} & 3485.2 & 3760.4 & 3520 & 3678.1 & 3511.2 & 3280.4 & 3098.7 \\
      &       & (1142.7) & (1456.1) & (1138.6) & (1322.6) & (949.9) & (941.9) & (948.4) \\
      & \multirow{2}[0]{*}{10} & 1081.5 & 2547 & 1479.3 & 1445.8 & 329.9 & 936.9 & 1039.2 \\
      &       & (405.4) & (479.8) & (421.6) & (433.3) & (458.5) & (433.7) & (445) \\
& & & & & & & & \\
\multirow{8}[0]{*}{10} & \multirow{2}[0]{*}{7} & 425.9 & 1337.6 & 837.6 & 782.6 & 484.9 & -1491.7 & -2302.2 \\
      &       & (1274.9) & (1227.3) & (1159) & (1203.6) & (1238.5) & (2223.3) & (2479.3) \\
      & \multirow{2}[0]{*}{8} & 430.1 & 242.8 & 392.6 & 332.8 & 428.8 & 235.4 & 194.6 \\
      &       & (1013.1) & (1054.8) & (1029.2) & (1030.2) & (1010.5) & (1019.2) & (1028) \\
      & \multirow{2}[0]{*}{9} & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
      &       & - & - & - & - & - & - & - \\
      & \multirow{2}[0]{*}{10} & 2861.6 & 3742 & 3515 & 3408.2 & 2935.4 & 2690.2 & 2433.4 \\
      &       & (982.7) & (987.2) & (957.1) & (980.3) & (986.8) & (1260.2) & (1327.7) \\
\midrule
\bottomrule
\end{tabular}


==> tables/hrs/attgt_results.tex <==
\begin{tabular}{cccccccc}
\toprule
\midrule
\makecell{Wave first \\ hospitalized} & Wave & Const. & \makecell{Doubly \\ robust} & \makecell{Non-orthogonal $\psi$ \\ No Sample splitting} & \makecell{Orthogonal $\psi^*$ \\ No sample splitting} & \makecell{Non-orthogonal $\psi$ \\ With sample splitting} & DML
 \\
      &       & (1)   & (2)   & (3)   & (4)   & (5)   & (6) \\ \midrule
\multirow{8}[0]{*}{8} & \multirow{2}[0]{*}{7} & 0 & 0 & 0 & 0 & 0 & 0 \\
      &       & - & - & - & - & - & - \\
      & \multirow{2}[0]{*}{8} & 3028.6 & 2200.5 & 2593.1 & 2480.2 & 2631.8 & 2521 \\
      &       & (913.5) & (839) & (689) & (788.3) & (689.7) & (799.6) \\
      & \multirow{2}[0]{*}{9} & 1247.7 & -14.3 & 1064 & 823.9 & 1022.2 & 534.3 \\
      &       & (860.7) & (681) & (439.5) & (505.8) & (441.3) & (592.6) \\
      & \multirow{2}[0]{*}{10} & 800.1 & 998.9 & 937.8 & 875.2 & 903.4 & 685 \\
      &       & (1007.5) & (570.2) & (508.2) & (513.4) & (508.7) & (603) \\
& & & & & & & \\
\multirow{8}[0]{*}{9} & \multirow{2}[0]{*}{7} & 170 & 1717.8 & 593.6 & 909 & 650.5 & 930.9 \\
      &       & (1128.4) & (1324.8) & (578.9) & (1123.4) & (580.3) & (1149) \\
      & \multirow{2}[0]{*}{8} & 0 & 0 & 0 & 0 & 0 & 0 \\
      &       & - & - & - & - & - & - \\
      & \multirow{2}[0]{*}{9} & 3324.4 & 3789.9 & 3324.4 & 3556.7 & 3324.4 & 3485.2 \\
      &       & (958.8) & (1338.6) & (643.5) & (1184.8) & (644.1) & (1142.7) \\
      & \multirow{2}[0]{*}{10} & 106.8 & 2533.6 & 887.7 & 1014.9 & 891 & 1081.5 \\
      &       & (650.7) & (421.7) & (370.7) & (384) & (372.4) & (405.4) \\
& & & & & & & \\
\multirow{8}[0]{*}{10} & \multirow{2}[0]{*}{7} & 591 & 1221.5 & 591 & 475.3 & 590 & 425.9 \\
      &       & (1268.9) & (1126.7) & (987.2) & (1217.3) & (989.3) & (1274.9) \\
      & \multirow{2}[0]{*}{8} & 410.6 & 246.7 & 413.5 & 434.7 & 410.3 & 430.1 \\
      &       & (1027.1) & (1026.2) & (987.7) & (1009.1) & (989.1) & (1013.1) \\
      & \multirow{2}[0]{*}{9} & 0 & 0 & 0 & 0 & 0 & 0 \\
      &       & - & - & - & - & - & - \\
      & \multirow{2}[0]{*}{10} & 3091.5 & 3796.1 & 3002.7 & 2991.9 & 2994.6 & 2861.6 \\
      &       & (995.4) & (931.6) & (834.3) & (907.8) & (836) & (982.7) \\
\midrule
\bottomrule
\end{tabular}


==> tables/hrs/calibration_factors/calib_lasso.tex <==
\begin{tabular}{cccccccc}
\toprule \midrule
& & \multicolumn{5}{c}{\it Cross-fitting Repetitions} & \\
\cmidrule(lr){3-7}
\makecell{Wave first \\ hospitalized} & Wave & Rep.\ 1 & Rep.\ 2 & Rep.\ 3 & Rep.\ 4 & Rep.\ 5 & \makecell{Median \\ aggregate} \\
& & (1) & (2) & (3) & (4) & (5) & (6) \\
\midrule
\multirow{4}{*}{8} & 7 & - & - & - & - & - & - \\
      & 8 & 0.111 & 0.064 & -0.024 & -0.107 & 0.032 & 0.032 \\
      & 9 & 0.081 & 0.131 & 0.091 & 0.044 & 0.07 & 0.081 \\
      & 10 & 0 & 0.003 & 0 & 0 & -0.001 & 0 \\
& & & & & & & \\
\multirow{4}{*}{9} & 7 & -0.669 & -0.547 & -0.481 & -0.826 & -0.554 & -0.554 \\
      & 8 & - & - & - & - & - & - \\
      & 9 & -1.828 & -1.516 & -0.98 & -1.854 & -0.895 & -1.516 \\
      & 10 & 0.002 & 0 & 0.001 & 0.001 & 0.002 & 0.001 \\
& & & & & & & \\
\multirow{4}{*}{10} & 7 & 0.17 & 0.218 & 0.105 & 0.292 & 0.142 & 0.17 \\
      & 8 & -1.507 & -1.492 & -1.83 & -1.499 & -1.966 & -1.507 \\
      & 9 & - & - & - & - & - & - \\
      & 10 & 0.055 & 0.019 & 0.154 & -0.1 & -0.114 & 0.019 \\
\midrule
\bottomrule
\end{tabular}


==> tables/hrs/calibration_factors/calib_linear.tex <==
\begin{tabular}{cccccccc}
\toprule \midrule
& & \multicolumn{5}{c}{\it Cross-fitting Repetitions} & \\
\cmidrule(lr){3-7}
\makecell{Wave first \\ hospitalized} & Wave & Rep.\ 1 & Rep.\ 2 & Rep.\ 3 & Rep.\ 4 & Rep.\ 5 & \makecell{Median \\ aggregate} \\
& & (1) & (2) & (3) & (4) & (5) & (6) \\
\midrule
\multirow{4}{*}{8} & 7 & - & - & - & - & - & - \\
      & 8 & 0.193 & 0.139 & 0.105 & 0.13 & 0.179 & 0.139 \\
      & 9 & 0.016 & -0.006 & 0.014 & 0.02 & 0.022 & 0.016 \\
      & 10 & 0 & 0 & 0 & 0 & 0 & 0 \\
& & & & & & & \\
\multirow{4}{*}{9} & 7 & -0.051 & -0.085 & -0.063 & -0.098 & -0.09 & -0.085 \\
      & 8 & - & - & - & - & - & - \\
      & 9 & -0.518 & -0.323 & -0.376 & -0.356 & -0.435 & -0.376 \\
      & 10 & 0.001 & 0.001 & 0.001 & 0 & 0.001 & 0.001 \\
& & & & & & & \\
\multirow{4}{*}{10} & 7 & 0.122 & 0.066 & 0.116 & 0.113 & 0.047 & 0.113 \\
      & 8 & 1.055 & 0.9 & 0.758 & 0.611 & 1.015 & 0.9 \\
      & 9 & - & - & - & - & - & - \\
      & 10 & 0.064 & -0.096 & 0.048 & 0.017 & 0.008 & 0.017 \\
\midrule
\bottomrule
\end{tabular}


==> tables/hrs/calibration_factors/calib_ranger1.tex <==
\begin{tabular}{cccccccc}
\toprule \midrule
& & \multicolumn{5}{c}{\it Cross-fitting Repetitions} & \\
\cmidrule(lr){3-7}
\makecell{Wave first \\ hospitalized} & Wave & Rep.\ 1 & Rep.\ 2 & Rep.\ 3 & Rep.\ 4 & Rep.\ 5 & \makecell{Median \\ aggregate} \\
& & (1) & (2) & (3) & (4) & (5) & (6) \\
\midrule
\multirow{4}{*}{8} & 7 & - & - & - & - & - & - \\
      & 8 & 0.542 & 0.561 & 0.529 & 0.631 & 0.493 & 0.542 \\
      & 9 & 0.203 & 0.219 & 0.132 & 0.205 & 0.228 & 0.205 \\
      & 10 & -0.132 & -0.234 & -0.037 & -0.337 & -0.39 & -0.234 \\
& & & & & & & \\
\multirow{4}{*}{9} & 7 & 0.061 & 0.249 & 0.239 & 0.076 & 0.129 & 0.129 \\
      & 8 & - & - & - & - & - & - \\
      & 9 & -0.636 & -0.69 & -0.769 & -0.771 & -0.749 & -0.749 \\
      & 10 & -0.195 & -0.172 & -0.194 & -0.23 & -0.214 & -0.195 \\
& & & & & & & \\
\multirow{4}{*}{10} & 7 & 0.275 & 0.294 & 0.257 & 0.362 & 0.356 & 0.294 \\
      & 8 & -1.325 & -1.157 & -1.1 & -1.325 & -0.944 & -1.157 \\
      & 9 & - & - & - & - & - & - \\
      & 10 & 0.251 & 0.315 & 0.169 & 0.285 & 0.279 & 0.279 \\
\midrule
\bottomrule
\end{tabular}


==> tables/hrs/calibration_factors/calib_ranger2.tex <==
\begin{tabular}{cccccccc}
\toprule \midrule
& & \multicolumn{5}{c}{\it Cross-fitting Repetitions} & \\
\cmidrule(lr){3-7}
\makecell{Wave first \\ hospitalized} & Wave & Rep.\ 1 & Rep.\ 2 & Rep.\ 3 & Rep.\ 4 & Rep.\ 5 & \makecell{Median \\ aggregate} \\
& & (1) & (2) & (3) & (4) & (5) & (6) \\
\midrule
\multirow{4}{*}{8} & 7 & - & - & - & - & - & - \\
      & 8 & 0.227 & 0.236 & 0.216 & 0.22 & 0.202 & 0.22 \\
      & 9 & -0.008 & -0.01 & -0.056 & -0.018 & 0.002 & -0.01 \\
      & 10 & 0.021 & -0.001 & 0.002 & 0.005 & -0.001 & 0.002 \\
& & & & & & & \\
\multirow{4}{*}{9} & 7 & -0.051 & 0.002 & 0.004 & -0.066 & -0.063 & -0.051 \\
      & 8 & - & - & - & - & - & - \\
      & 9 & -0.043 & -0.035 & -0.049 & -0.071 & -0.043 & -0.043 \\
      & 10 & 0.12 & 0.066 & 0.04 & 0.036 & 0.028 & 0.04 \\
& & & & & & & \\
\multirow{4}{*}{10} & 7 & 0.542 & 0.634 & 0.557 & 0.778 & 0.972 & 0.634 \\
      & 8 & 0.831 & 0.35 & 0.482 & 0.395 & 0.581 & 0.482 \\
      & 9 & - & - & - & - & - & - \\
      & 10 & 0.024 & -0.09 & -0.059 & -0.027 & 0.393 & -0.027 \\
\midrule
\bottomrule
\end{tabular}


==> tables/hrs/calibration_factors/calib_ranger3.tex <==
\begin{tabular}{cccccccc}
\toprule \midrule
& & \multicolumn{5}{c}{\it Cross-fitting Repetitions} & \\
\cmidrule(lr){3-7}
\makecell{Wave first \\ hospitalized} & Wave & Rep.\ 1 & Rep.\ 2 & Rep.\ 3 & Rep.\ 4 & Rep.\ 5 & \makecell{Median \\ aggregate} \\
& & (1) & (2) & (3) & (4) & (5) & (6) \\
\midrule
\multirow{4}{*}{8} & 7 & - & - & - & - & - & - \\
      & 8 & 0.179 & 0.189 & 0.172 & 0.181 & 0.155 & 0.179 \\
      & 9 & -0.034 & -0.033 & -0.114 & -0.04 & -0.04 & -0.04 \\
      & 10 & -0.012 & -0.048 & -0.043 & -0.013 & -0.032 & -0.032 \\
& & & & & & & \\
\multirow{4}{*}{9} & 7 & -0.017 & 0.011 & 0.012 & -0.019 & -0.05 & -0.017 \\
      & 8 & - & - & - & - & - & - \\
      & 9 & -0.015 & -0.015 & -0.023 & -0.046 & -0.004 & -0.015 \\
      & 10 & 0.102 & 0.079 & 0.042 & 0.058 & 0.046 & 0.058 \\
& & & & & & & \\
\multirow{4}{*}{10} & 7 & 0.572 & 0.709 & 0.462 & 0.573 & 1.04 & 0.573 \\
      & 8 & 0.937 & 0.286 & 0.391 & 0.368 & 0.39 & 0.39 \\
      & 9 & - & - & - & - & - & - \\
      & 10 & 0.221 & 0.065 & 0.091 & 0.192 & 0.399 & 0.192 \\
\midrule
\bottomrule
\end{tabular}


==> tables/hrs/calibration_factors/calib_ridge.tex <==
\begin{tabular}{cccccccc}
\toprule \midrule
& & \multicolumn{5}{c}{\it Cross-fitting Repetitions} & \\
\cmidrule(lr){3-7}
\makecell{Wave first \\ hospitalized} & Wave & Rep.\ 1 & Rep.\ 2 & Rep.\ 3 & Rep.\ 4 & Rep.\ 5 & \makecell{Median \\ aggregate} \\
& & (1) & (2) & (3) & (4) & (5) & (6) \\
\midrule
\multirow{4}{*}{8} & 7 & - & - & - & - & - & - \\
      & 8 & 0.007 & 0.158 & 0.043 & -0.09 & -0.062 & 0.007 \\
      & 9 & 0.142 & 0.23 & 0.231 & 0.109 & 0.161 & 0.161 \\
      & 10 & 0.001 & 0.004 & 0.004 & 0 & 0.003 & 0.003 \\
& & & & & & & \\
\multirow{4}{*}{9} & 7 & -1.096 & -1.191 & -0.686 & -1.24 & -1.185 & -1.185 \\
      & 8 & - & - & - & - & - & - \\
      & 9 & -1.682 & -0.851 & -1.304 & -1.689 & -1.151 & -1.304 \\
      & 10 & 0.002 & -0.022 & 0.001 & -0.003 & -0.007 & -0.003 \\
& & & & & & & \\
\multirow{4}{*}{10} & 7 & 0.096 & 0.337 & 0.115 & 0.377 & 0.202 & 0.202 \\
      & 8 & -0.528 & -1.817 & -1.346 & -1.414 & -1.333 & -1.346 \\
      & 9 & - & - & - & - & - & - \\
      & 10 & 0.084 & 0.02 & -0.051 & -0.214 & -0.271 & -0.051 \\
\midrule
\bottomrule
\end{tabular}


==> tables/hrs/calibration_factors/calib_stack.tex <==
\begin{tabular}{cccccccc}
\toprule \midrule
& & \multicolumn{5}{c}{\it Cross-fitting Repetitions} & \\
\cmidrule(lr){3-7}
\makecell{Wave first \\ hospitalized} & Wave & Rep.\ 1 & Rep.\ 2 & Rep.\ 3 & Rep.\ 4 & Rep.\ 5 & \makecell{Median \\ aggregate} \\
& & (1) & (2) & (3) & (4) & (5) & (6) \\
\midrule
\multirow{4}{*}{8} & 7 & - & - & - & - & - & - \\
      & 8 & 0.428 & 0.439 & 0.612 & 0.571 & 0.569 & 0.569 \\
      & 9 & 0.072 & 0.311 & 0.169 & 0.122 & 0.144 & 0.144 \\
      & 10 & -0.025 & -0.256 & -1.575 & 0.001 & -0.025 & -0.025 \\
& & & & & & & \\
\multirow{4}{*}{9} & 7 & -0.377 & -0.417 & -0.572 & 0.125 & -0.03 & -0.377 \\
      & 8 & - & - & - & - & - & - \\
      & 9 & -1.135 & -1.244 & -1.437 & -1.246 & -0.771 & -1.244 \\
      & 10 & 0.019 & 0.012 & 0.016 & 0.017 & 0.02 & 0.017 \\
& & & & & & & \\
\multirow{4}{*}{10} & 7 & 0.193 & 0.235 & 0.391 & 0.251 & 0.282 & 0.251 \\
      & 8 & -1.966 & -1.516 & -0.798 & -1.835 & -1.201 & -1.516 \\
      & 9 & - & - & - & - & - & - \\
      & 10 & 0.73 & 0.746 & 0.655 & 0.6 & 0.598 & 0.655 \\
\midrule
\bottomrule
\end{tabular}


==> tables/hrs/dyn_bylearner.tex <==
\begin{tabular}{cccccccc}
\toprule
\midrule
\makecell{Relative \\ Event Time} & \makecell{Short- \\ stacking} & \makecell{Linear \\ index} & Lasso & Ridge & \makecell{Random \\ Forest (hr)} & \makecell{Random \\ Forest (mr)} & \makecell{Random \\ Forest (lr)}
 \\
      & (1)   & (2)   & (3)   & (4)   & (5)   & (6) & (7) \\ \midrule
-3 & 425.9 & 1337.6 & 837.6 & 782.6 & 484.9 & -1491.7 & -2302.2 \\
      & (1274.9) & (1227.3) & (1159) & (1203.6) & (1238.5) & (2223.3) & (2479.3) \\
-2 & 690.1 & 949.4 & 690.3 & 740.8 & 676.5 & 819.7 & 861.7 \\
      & (1003.8) & (1168.2) & (1013.5) & (1098.6) & (900.2) & (889.5) & (871.9) \\
-1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
      & - & - & - & - & - & - & - \\
0 & 2924.3 & 3169.6 & 2994.9 & 3042.7 & 2903.3 & 2758.3 & 2665.6 \\
      & (518) & (559) & (495.2) & (529.5) & (496.5) & (554.2) & (570.9) \\
1 & 788.6 & 1072.8 & 1066.1 & 1013.8 & 578.4 & 678.1 & 667.2 \\
      & (392.2) & (479.7) & (405.2) & (413.2) & (380) & (404.9) & (425) \\
2 & 685 & 898.8 & 872.6 & 856.8 & 769.6 & 723.7 & 623.6 \\
      & (603) & (638.1) & (518) & (519.2) & (588.5) & (599.9) & (626.8) \\
\midrule
\bottomrule
\end{tabular}


==> tables/hrs/dyn_ranger2.tex <==
\begin{tabular}{cccccccccc}
\toprule \midrule
& & & \multicolumn{5}{c}{\it Cross-fitting Repetitions} & \\
\cmidrule(lr){4-8}
\makecell{Relative \\ Event Time} & Const.\ & \makecell{Doubly \\ robust} & Rep.\ 1 & Rep.\ 2 & Rep.\ 3 & Rep.\ 4 & Rep.\ 5 & \makecell{Median \\ aggregate}\\
\midrule
\multirow{2}[0]{*}{-3} & 591 & 1221.5 & -1248 & -1783.6 & -1856.9 & -577.4 & -1491.7 & -1491.7 \\
      & (1268.9) & (1126.7) & (2203.2) & (2473.6) & (2624.7) & (1661.1) & (2223.3) & (2223.3) \\
\multirow{2}[0]{*}{-2} & 285.7 & 1010.5 & 849.7 & 819.7 & 840.4 & 805.3 & 788.1 & 819.7 \\
      & (946.8) & (1105.2) & (913.4) & (889.5) & (889.4) & (874.3) & (868.6) & (889.5) \\
\multirow{2}[0]{*}{-1} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
      & - & - & - & - & - & - & - & - \\
\multirow{2}[0]{*}{0} & 3134 & 3113.9 & 2843.4 & 2781.1 & 2742 & 2758.3 & 2731.9 & 2758.3 \\
      & (535.7) & (533.8) & (546.2) & (539.1) & (554.4) & (570) & (553.6) & (554.2) \\
\multirow{2}[0]{*}{1} & 778.6 & 1033.4 & 773.3 & 659.6 & 765 & 659.6 & 678.1 & 678.1 \\
      & (569.7) & (443) & (390.4) & (409.2) & (395.5) & (418.3) & (389.1) & (404.9) \\
\multirow{2}[0]{*}{2} & 800.1 & 998.9 & 723.7 & 803 & 766.6 & 614.8 & 691.8 & 723.7 \\
      & (1007.5) & (570.2) & (582.6) & (580.9) & (598.3) & (599.3) & (616.3) & (599.9) \\
\midrule
\bottomrule
\end{tabular}


==> tables/hrs/dyn_results.tex <==
\begin{tabular}{ccccccc}
\toprule
\midrule
\makecell{Relative \\ Event Time} & Const. & \makecell{Doubly \\ robust} & \makecell{Non-orthogonal $\psi$ \\ No Sample splitting} & \makecell{Orthogonal $\psi^*$ \\ No sample splitting} & \makecell{Non-orthogonal $\psi$ \\ With sample splitting} & DML
 \\
      & (1)   & (2)   & (3)   & (4)   & (5)   & (6) \\ \midrule
-3 & 591 & 1221.5 & 591 & 475.3 & 590 & 425.9 \\
      & (1268.9) & (1126.7) & (987.2) & (1217.3) & (989.3) & (1274.9) \\
-2 & 285.7 & 1010.5 & 507 & 680.9 & 535 & 690.1 \\
      & (946.8) & (1105.2) & (562) & (989.7) & (563.7) & (1003.8) \\
-1 & 0 & 0 & 0 & 0 & 0 & 0 \\
      & - & - & - & - & - & - \\
0 & 3134 & 3113.9 & 2923.9 & 2941.9 & 2939.6 & 2924.3 \\
      & (535.7) & (533.8) & (419.7) & (509.1) & (420.2) & (518) \\
1 & 778.6 & 1033.4 & 991.5 & 902.4 & 973.3 & 788.6 \\
      & (569.7) & (443) & (300.4) & (337.1) & (301.6) & (392.2) \\
2 & 800.1 & 998.9 & 937.8 & 875.2 & 903.4 & 685 \\
      & (1007.5) & (570.2) & (508.2) & (513.4) & (508.7) & (603) \\
\midrule
\bottomrule
\end{tabular}


==> tables/hrs/groups.tex <==
\begin{tabular}{ccccc}
\toprule \midrule
\makecell{Wave first \\ hospitalized} & Wave & \makecell{Treated \\ Observations} & \makecell{Control \\ Observations} & \makecell{Trimmed \\ observations}
 \\
\midrule
\multirow{3}{*}{8} & 7 & - & - & - \\
      & 8 & 252 & 404 & 0 \\
      & 9 & 252 & 228 & 0 \\
      & 10 & 252 & 65 & 0 \\
\midrule
\multirow{3}{*}{9} & 7 & 176 & 228 & 0 \\
      & 8 & - & - & - \\
      & 9 & 176 & 228 & 0 \\
      & 10 & 176 & 65 & 0 \\
\midrule
\multirow{3}{*}{10} & 7 & 163 & 65 & 0 \\
      & 8 & 163 & 65 & 0 \\
      & 9 & - & - & - \\
      & 10 & 163 & 65 & 0 \\
\midrule \bottomrule
\end{tabular}


==> tables/hrs/mspe_bylearner.tex <==
\begin{tabular}{cccccccccc}
\toprule \midrule
\makecell{Wave first \\ hospitalized} & Wave &  & \makecell{Short- \\ stacking} & \makecell{Linear \\ index} & Lasso & Ridge & \makecell{Random \\ Forest (hr)} & \makecell{Random \\ Forest (mr)} & \makecell{Random \\ Forest (lr)}
 \\
      &       &       & (1)   & (2)   & (3)   & (4)   & (5)   & (6)   & (7) \\ \midrule
\multirow{12}{*}{8} & \multirow{4}{*}{8} & RMSPE (y) & 12.118 & 12.192 & 12.154 & 12.155 & 12.104 & 12.307 & 12.518 \\
      &       & RMSPE (D) & 0.455 & 0.462 & 0.46 & 0.461 & 0.455 & 0.456 & 0.457 \\
      &       & Weights (y) & - & 0 & 0 & 0.2 & 0.8 & 0 & 0 \\
      &       & Weights (D) & - & 0 & 0 & 0 & 0.6 & 0.4 & 0 \\
& & & & & & & & & \\
      & \multirow{4}{*}{9} & RMSPE (y) & 11.199 & 11.409 & 11.274 & 11.274 & 11.153 & 11.4 & 11.775 \\
      &       & RMSPE (D) & 0.43 & 0.439 & 0.433 & 0.436 & 0.436 & 0.432 & 0.432 \\
      &       & Weights (y) & - & 0 & 0 & 0.2 & 0.8 & 0 & 0 \\
      &       & Weights (D) & - & 0 & 0.4 & 0 & 0 & 0 & 0.6 \\
& & & & & & & & & \\
      & \multirow{4}{*}{10} & RMSPE (y) & 7.014 & 7.769 & 7.202 & 7.169 & 7.185 & 7.283 & 7.136 \\
      &       & RMSPE (D) & 0.341 & 0.353 & 0.343 & 0.347 & 0.355 & 0.343 & 0.342 \\
      &       & Weights (y) & - & 0 & 0 & 0 & 0 & 0 & 1 \\
      &       & Weights (D) & - & 0 & 0.4 & 0 & 0 & 0 & 0.6 \\
& & & & & & & & & \\
\multirow{12}{*}{9} & \multirow{4}{*}{7} & RMSPE (y) & 14.706 & 14.938 & 14.803 & 14.761 & 14.67 & 14.927 & 15.322 \\
      &       & RMSPE (D) & 0.436 & 0.441 & 0.436 & 0.44 & 0.446 & 0.442 & 0.443 \\
      &       & Weights (y) & - & 0 & 0 & 0.2 & 0.8 & 0 & 0 \\
      &       & Weights (D) & - & 0 & 1 & 0 & 0 & 0 & 0 \\
& & & & & & & & & \\
      & \multirow{4}{*}{9} & RMSPE (y) & 10.784 & 11.032 & 10.793 & 10.789 & 10.856 & 11.099 & 11.291 \\
      &       & RMSPE (D) & 0.442 & 0.446 & 0.442 & 0.445 & 0.449 & 0.449 & 0.451 \\
      &       & Weights (y) & - & 0 & 0.4 & 0.6 & 0 & 0 & 0 \\
      &       & Weights (D) & - & 0 & 1 & 0 & 0 & 0 & 0 \\
& & & & & & & & & \\
      & \multirow{4}{*}{10} & RMSPE (y) & 4.064 & 4.399 & 4.468 & 4.412 & 4.4 & 4.246 & 4.215 \\
      &       & RMSPE (D) & 0.375 & 0.387 & 0.374 & 0.379 & 0.388 & 0.383 & 0.385 \\
      &       & Weights (y) & - & 0 & 0 & 0 & 0 & 0 & 1 \\
      &       & Weights (D) & - & 0 & 1 & 0 & 0 & 0 & 0 \\
& & & & & & & & & \\
\multirow{12}{*}{10} & \multirow{4}{*}{7} & RMSPE (y) & 6.55 & 6.917 & 6.539 & 6.549 & 6.549 & 6.575 & 6.574 \\
      &       & RMSPE (D) & 0.435 & 0.457 & 0.447 & 0.453 & 0.435 & 0.444 & 0.45 \\
      &       & Weights (y) & - & 0 & 0.4 & 0 & 0.4 & 0 & 0.2 \\
      &       & Weights (D) & - & 0 & 0 & 0 & 1 & 0 & 0 \\
& & & & & & & & & \\
      & \multirow{4}{*}{8} & RMSPE (y) & 2.312 & 2.439 & 2.322 & 2.327 & 2.312 & 2.372 & 2.403 \\
      &       & RMSPE (D) & 0.434 & 0.457 & 0.448 & 0.454 & 0.433 & 0.443 & 0.451 \\
      &       & Weights (y) & - & 0 & 0 & 0 & 1 & 0 & 0 \\
      &       & Weights (D) & - & 0 & 0 & 0 & 1 & 0 & 0 \\
& & & & & & & & & \\
      & \multirow{4}{*}{10} & RMSPE (y) & 4.439 & 4.653 & 4.701 & 4.662 & 4.594 & 4.541 & 4.657 \\
      &       & RMSPE (D) & 0.433 & 0.457 & 0.448 & 0.453 & 0.432 & 0.436 & 0.442 \\
      &       & Weights (y) & - & 0 & 0 & 0 & 0 & 0.8 & 0.2 \\
      &       & Weights (D) & - & 0 & 0 & 0 & 1 & 0 & 0 \\
\midrule \bottomrule
\end{tabular}


==> tables/scores_overview.tex <==
\begin{table*}[htbp]
\newcommand{\mybm}[1]{#1}
\scriptsize
\begin{tabularx}{\linewidth}{l>{\raggedright}p{.22\linewidth}X} \toprule\toprule
\multicolumn{2}{l}{Assumptions} & Neyman-orthogonal score \\  \midrule 
\multicolumn{3}{l}{\bfseries Partially Linear Model} \\ 
&
\noindent\parbox[c]{\hsize}{\raggedright%
A1. Conditional orthogonality $E[Cov(U, D\vert \mybm{X})]= 0$ \newline 
A2. $E[Var(D\vert \mybm{X})] \neq 0$
} 
&
$\displaystyle\psi(\mybm{W}; \alpha_{\textnormal{PLM}}, m,\ell) = \Big(Y - \ell(\mybm{X}) - \alpha_{\textnormal{PLM}}\big(D - m(\mybm{X})\big)\Big)\big(D - m(\mybm{X})\big)$
\\ 
 && \\
\multicolumn{3}{l}{\bfseries Interactive Model}  \\
&
\noindent\parbox[c]{\hsize}{\raggedright%
A3. Conditional Mean Independence $E[U\vert D, \mybm{X}]=0$  \newline
A4. Overlap $\Pr(D=1 \vert \mybm{X})\in (0,1)$  % with probability 1.
}
&
$\displaystyle\psi(\mybm{W};\alpha_{\textnormal{ATE}}, g, m) =  \frac{D(Y-g(1, \mybm{X}))}{m(\mybm{X})} {-} \frac{(1-D)(Y - g(0, \mybm{X}))}{1 - m(\mybm{X})} {+} g(1, \mybm{X}) {-} g(0, \mybm{X}) {-} \alpha_{\textnormal{ATE}}$ \newline  $\displaystyle\psi(\mybm{W};\alpha_{\textnormal{ATET}}, g, m, p) =  \frac{D(Y - g(0,\mybm{X}))}{p} - \frac{m(\mybm{X})(1-D)(Y-g(0,\mybm{X}))}{p(1-m(\mybm{X}))} -  \frac{D\alpha_{\textnormal{ATET}}}{p} $
\\
&& \\
\multicolumn{3}{l}{\bfseries Partially Linear IV Model}\\
&
\noindent\parbox[c]{\hsize}{\raggedright%
A5. Conditional IV Orthogonality $E[Cov(U,Z\vert \mybm{X})]= 0$. \newline
A6. Conditional Linear IV Relevance $E[Cov(D,Z\vert \mybm{X})]\neq 0$.
}
&
$\displaystyle\psi(\mybm{W}; \alpha_{\textnormal{IV}}, \ell,m,r) = \Big(Y-\ell(\mybm{X}) - \alpha_{\textnormal{IV}}(D - m(\mybm{X}))\Big)\Big(Z - r(\mybm{X})\Big)$ 
\\
 && \\
\multicolumn{3}{l}{\bfseries Flexible Partially Linear IV Model} \\
&
\noindent\parbox[c]{\hsize}{\raggedright%
A7. Conditional IV Mean Independence
$E[U\vert \mybm{Z},\mybm{X}] = 0$. \newline
A8. Conditional IV Relevance
$E[Var(E[D\vert \mybm{Z},\mybm{X}]\vert \mybm{X})] \neq 0.$ 
}
&
$  \displaystyle\psi(\mybm{W}; \alpha_{\textnormal{FIV}}, \ell, m, p) = \Big(Y-\ell(\mybm{X}) - \alpha_{\textnormal{FIV}}(D - m(\mybm{X}))\Big)\Big(p(\mybm{Z}, \mybm{X}) - m(\mybm{X})\Big) $ 
\\
 && \\
\multicolumn{3}{l}{\bfseries Interactive IV Model} \\
&
\noindent\parbox[c]{\hsize}{\raggedright%
A7., A8., and \newline
A9. Monotonicity $p_0(1, \mybm{X})\geq p_0(0, \mybm{X})$ \newline 
A10. Overlap $\Pr(Z=1\vert \mybm{X})\in(0,1)$ 
}
&
$\displaystyle\psi(\mybm{W};\alpha_{\textnormal{LATE}}, g, m) =  \frac{E\left[\ell_0(1, \mybm{X})-\ell_0(0, \mybm{X})\right]}{E\left[p_0(1, \mybm{X})-p_0(0, \mybm{X})\right]} - \alpha_{\textnormal{LATE}}$
\\ 
\bottomrule\bottomrule
\end{tabularx}\par\medskip
\parbox{\linewidth}{{\it Notes:} $m_0(\mybm{X})\equiv E[D\vert \mybm{X}] $ and $\ell_0(\mybm{X})\equiv E[Y\vert \mybm{X}]$; $g_0(D,\mybm{X})\equiv E[Y\vert D, \mybm{X}]$, and $p_0 \equiv E[D]$, and $r_0(\mybm{X})\equiv E[Z\vert \mybm{X}]$.}
\caption{Overview of Neyman-orthogonal score functions}
\label{tab:overview_scores}
\end{table*}

==> tables/scores_overview_2.tex <==
\begin{tabularx}{\linewidth}{l>{\raggedright}p{.22\linewidth}X} \toprule\toprule \\
\multicolumn{3}{l}{\bfseries Partially Linear Regression Coefficient} \\
$W \equiv (Y, D, X); $\\ 
$\eta \equiv (m, \ell) \text{ where } m_0(X) \equiv \Ep[D\vert X], \:\ell_0(X) \equiv \Ep[Y\vert X]; $\\
$\psi^a(W; \eta) \equiv -(D - m(X))^2; $\\
$\psi^b(W; \eta) \equiv (Y - \ell(X))(D - m(X));$
\\ && \\

\multicolumn{3}{l}{\bfseries Average Treatment Effect}  \\
$W \equiv (Y, D, X);$ \\
$\eta \equiv (m, g^{(0)}, g^{(1)}) \text{ where } m_0(X) \equiv \Ep[D\vert X], \:g^{(d)}_0(X) \equiv \Ep[Y\vert D=0, X], \: d \in \{0,1\}; $ \\
$\psi^a(W; \eta) \equiv -1; $\\
$\psi^b(W; \eta) \equiv \frac{D(Y-g^{(1)}(\mybm{X}))}{m(\mybm{X})} {-} \frac{(1-D)(Y - g^{(0)}(\mybm{X}))}{1 - m(\mybm{X})} {+} g^{(1)}(\mybm{X}) {-} g^{(0)}(\mybm{X});$
\\ && \\

\multicolumn{3}{l}{\bfseries Average Treatment Effect on the Treated}  \\
$W \equiv (Y, D, X); $\\
$\eta \equiv (m, g^{(0)}, p) \text{ where } m_0(X) \equiv \Ep[D\vert X], \:g^{(0)}_0(X) \equiv \Ep[Y\vert D=0, X],\: p_0 \equiv \Ep[D] ;$\\
$\psi^a(W; \eta) \equiv -\frac{D}{p};$ \\
$\psi^b(W; \eta) \equiv \frac{D(Y - g^{(0)}(\mybm{X}))}{p} - \frac{m(\mybm{X})(1-D)(Y-g^{(0)}(\mybm{X}))}{p(1-m(\mybm{X}))};$
\\ && \\

\multicolumn{3}{l}{\bfseries Partially Linear IV Regression Coefficient}\\
$W \equiv (Y, D, X, Z); $\\ 
$\eta \equiv (m, \ell, r) \text{ where } m_0(X) \equiv \Ep[D\vert X], \:\ell_0(X) \equiv \Ep[Y\vert X]; \: r_0(X) \equiv \Ep[Z\vert X];$\\
$\psi^a(W; \eta) \equiv -(D - m(X))(Z - r(X)); $\\
$\psi^b(W; \eta) \equiv (Y - \ell(X))(Z - r(X));$
\\ && \\

\multicolumn{3}{l}{\bfseries Flexible Partially Linear IV Regression Coefficient} \\
$W \equiv (Y, D, X, Z);$ \\ 
$\eta \equiv (m, \ell, p) \text{ where } m_0(X) \equiv \Ep[D\vert X], \:\ell_0(X) \equiv \Ep[Y\vert X]; \: p_0(Z, X) \equiv \Ep[D\vert Z, X];$\\
$\psi^a(W; \eta) \equiv -(D - m(X))(p(Z,X) - m(X)); $\\
$\psi^b(W; \eta) \equiv (Y - \ell(X))(p(Z,X) - m(X));$
\\ && \\

\multicolumn{3}{l}{\bfseries Local Average Treatment Effect} \\
$W \equiv (Y, D, X, Z); $\\
$\eta \equiv (r, \ell^{(0)}, \ell^{(1)}, p^{(0)}, p^{(1)}) \text{ where }  \: r_0(X) \equiv \Ep[Z\vert X], \:\ell^{(z)}_0(X) \equiv \Ep[Y\vert Z=z, X], \:p^{(z)}_0(X) \equiv \Ep[D\vert Z=z, X], \: z \in \{0,1\};$  \\
$\psi^a(W; \eta) \equiv -\left(\frac{Z(D-p^{(1)}(\mybm{X}))}{r(\mybm{X})} {-} \frac{(1-Z)(D - p^{(0)}(\mybm{X}))}{1 - r(\mybm{X})} {+} p^{(1)}(\mybm{X}) {-} p^{(0)}(\mybm{X})\right);$ \\
$\psi^b(W; \eta) \equiv \frac{Z(Y-\ell^{(1)}(\mybm{X}))}{r(\mybm{X})} {-} \frac{(1-Z)(Y - \ell^{(0)}(\mybm{X}))}{1 - r(\mybm{X})} {+} \ell^{(1)}(\mybm{X}) {-} \ell^{(0)}(\mybm{X});$
\\ && \\

\bottomrule\bottomrule
\end{tabularx} 

==> tables/scores_overview_final.tex <==
\begin{tabularx}{\linewidth}{l>{\raggedright}p{.22\linewidth}X} \toprule\toprule \\
\multicolumn{3}{l}{\bfseries Average Treatment Effect}  \\
$W_i \equiv (Y_i, D_i, X_i)$ \\
$\eta \equiv (m, g^{(0)}, g^{(1)}) \text{ where } m_0(X_i) \equiv \Ep[D_i\vert X_i], \:g^{(d)}_0(X_i) \equiv \Ep[Y_i\vert D_i=0, X_i], \: d \in \{0,1\} $ \\
$\psi^*(W_i; \theta, \eta) = \frac{D_i(Y_i-g^{(1)}(X_i))}{m(X_i)} {-} \frac{(1-D_i)(Y_i - g^{(0)}(X_i))}{1 - m(X_i)} {+} g^{(1)}(X_i) {-} g^{(0)}(X_i) - \theta$
\\ && \\

\multicolumn{3}{l}{\bfseries Average Treatment Effect on the Treated}  \\
$W_i \equiv (Y_i, D_i, X_i)$ \\
$\eta \equiv (m, g^{(0)}, p) \text{ where } m_0(X_i) \equiv \Ep[D_i\vert X_i], \:g^{(0)}_0(X_i) \equiv \Ep[Y_i\vert D_i=0, X_i],\: p_0 \equiv \Ep[D_i] $\\
$\psi^*(W_i; \theta, \eta) \equiv \frac{D_i(Y_i - g^{(0)}(X_i))}{p} - \frac{m(X_i)(1-D_i)(Y_i-g^{(0)}(X_i))}{p(1-m(X_i))}  -\frac{D_i}{p}\theta$
\\ && \\

\multicolumn{3}{l}{\bfseries Partially Linear IV Regression Coefficient}\\
$W_i \equiv (Y_i, D_i, X_i, Z_i) $\\ 
$\eta \equiv (m, \ell, r) \text{ where } m_0(X_i) \equiv \Ep[D_i\vert X_i], \:\ell_0(X_i) \equiv \Ep[Y_i\vert X_i]; \: r_0(X_i) \equiv \Ep[Z_i\vert X_i]$\\
$\psi^*(W_i; \theta, \eta) \equiv (Y_i - \ell(X_i))(Z_i - r(X_i))-(D_i - m(X_i))(Z_i - r(X_i))\theta$

\\ && \\

\multicolumn{3}{l}{\bfseries Flexible Partially Linear IV Regression Coefficient} \\
$W_i \equiv (Y_i, D_i, X_i, Z_i)$ \\ 
$\eta \equiv (m, \ell, p) \text{ where } m_0(X_i) \equiv \Ep[D_i\vert X_i], \:\ell_0(X_i) \equiv \Ep[Y_i\vert X_i]; \: p_0(Z_i, X_i) \equiv \Ep[D_i\vert Z_i, X_i]$\\
$\psi^*(W_i; \theta, \eta) \equiv   (Y_i - \ell(X_i))(p(Z_i,X_i) - m(X_i)) -(D_i - m(X_i))(p(Z_i,X_i) - m(X_i))\theta$
\\ && \\

\multicolumn{3}{l}{\bfseries Local Average Treatment Effect} \\
$W_i \equiv (Y_i, D_i, X_i, Z_i) $\\ 
$\eta \equiv (r, \ell^{(0)}, \ell^{(1)}, p^{(0)}, p^{(1)}) \text{ where }  \: r_0(X_i) \equiv \Ep[Z_i\vert X_i], \:\ell^{(z)}_0(X_i) \equiv \Ep[Y_i\vert Z_i=z, X_i], \:p^{(z)}_0(X_i) \equiv \Ep[D_i\vert Z_i=z, X_i], \: z \in \{0,1\};$  \\
$\psi^*(W_i; \theta, \eta) \equiv  \frac{Z_i(Y_i-\ell^{(1)}(X_i))}{r(X_i)} {-} \frac{(1-Z_i)(Y_i - \ell^{(0)}(X_i))}{1 - r(X_i)} {+} \ell^{(1)}(X_i) {-} \ell^{(0)}(X_i)$ \\
$\qquad \qquad \qquad \qquad -\left(\frac{Z_i(D_i-p^{(1)}(X_i))}{r(X_i)} {-} \frac{(1-Z_i)(D_i - p^{(0)}(X_i))}{1 - r(X_i)} {+} p^{(1)}(X_i) {-} p^{(0)}(X_i)\right)\theta$
\\ && \\

\multicolumn{3}{l}{\bfseries Fixed Effects Partially Linear Regression Coefficient} \\
$W_{i}\equiv (Y_{it}, D_{it}, X_{it})_{t=0}^T$ and define $\Delta Y_{it}\equiv Y_{it}-Y_{it-1}, \Delta D_{it}\equiv D_{it}-D_{it-1}$\\
$\eta \equiv (m_{t}, \ell_t)_{t=1}^T$ where $m_{t0}(X_{it}, X_{it-1}) \equiv \Ep[\Delta D_{it}\vert X_{it}, X_{it-1}];\: \ell_{t0}(X_{it}, X_{it-1})\equiv \Ep[\Delta Y_{it}\vert X_{it}, X_{it-1}]$\ \\
$\psi^*(W_{i}; \theta, \eta) \equiv \sum_{t=1}^T\left(\Delta D_{it} - \Ep[\Delta D_{it}\vert X_{it},  X_{it-t}]\right)\left((\Delta Y_{it} - \Ep[\Delta Y_{it}\vert X_{it},  X_{it-t}]) - \theta(\Delta D_{it} - \Ep[\Delta D_{it}\vert X_{it},  X_{it-t}])\right)$
\\ && \\

\multicolumn{3}{l}{\bfseries Fixed Effects Partially Linear IV Regression Coefficient}\\
$W_{i}\equiv (Y_{it}, D_{it}, Z_{it}, X_{it})_{t=0}^T$ and define $\Delta Y_{it}\equiv Y_{it}-Y_{it-1}, \Delta D_{it}\equiv D_{it}-D_{it-1}, \Delta Z_{it}\equiv Z_{it}-Z_{it-1}$\\
$\eta \equiv (m_{t}, \ell_t, r_t)_{t=1}^T$ where $m_{t0}(X_{it}, X_{it-1}) \equiv \Ep[D_{it}\vert X_{it}, X_{it-1}];\: \ell_{t0}(X_{it}, X_{it-1})\equiv \Ep[Y_{it}\vert X_{it}, X_{it-1}];$\ \\
$\qquad  r_{t0}(X_{it}, X_{it-1})\equiv \Ep[\Delta Z_{it}\vert X_{it}, X_{it-1}]$ \\
$\psi^*(W_{i}; \theta, \eta) \equiv \sum_{t=1}^T\left(\Delta Z_{it} - \Ep[\Delta Z_{it}\vert X_{it},  X_{it-t}]\right)\left(\Delta Y_{it} - \Ep[\Delta Y_{it}\vert X_{it},  X_{it-t}]\right) $\\
$ \qquad \qquad \qquad \qquad - \sum_{t=1}^T \left(\Delta Z_{it} - \Ep[\Delta Z_{it}\vert X_{it},  X_{it-t}]\right)(\Delta D_{it} - \Ep[\Delta D_{it}\vert X_{it},  X_{it-t}])\theta$
\\ && \\
\bottomrule\bottomrule
\end{tabularx} 
